Bunny-VisionPro: Real-Time Bimanual Dexterous Teleoperation for Imitation Learning

Teleoperation is a crucial tool for collecting human demonstrations, but controlling robots with bimanual dexterous hands remains a challenge. Existing teleoperation systems struggle to handle the complexity of coordinating two hands for intricate manipulations. We introduce Bunny-VisionPro, a real-time bimanual dexterous teleoperation system that leverages a VR headset. Unlike previous vision-based teleoperation systems, we design novel low-cost devices to provide haptic feedback to the operator, enhancing immersion. Our system prioritizes safety by incorporating collision and singularity avoidance while maintaining real-time performance through innovative designs. Bunny-VisionPro outperforms prior systems on a standard task suite, achieving higher success rates and reduced task completion times. Moreover, the high-quality teleoperation demonstrations improve downstream imitation learning performance, leading to better generalizability. Notably, Bunny-VisionPro enables imitation learning with challenging multi-stage, long-horizon dexterous manipulation tasks, which have rarely been addressed in previous work. Our system's ability to handle bimanual manipulations while prioritizing safety and real-time performance makes it a powerful tool for advancing dexterous manipulation and imitation learning.

==> table/imitation_table_lh.tex <==
\begin{table}[]
\centering
\begin{small}
\setlength\tabcolsep{5pt}
\scalebox{1.0}{
\begin{tabular}{lccc}
\toprule
\multirow{2}{*}{Task} & \multicolumn{3}{c}{DP3~\citep{ze20243d}} \\
\cmidrule{2-3}
 &  SR-Subtask & SR & \\
 \midrule

Wipe Glass & 0.7 & 0.7 \\

\rowcolor{gray!10}
Sweep Floor  & & \\

Prepare Coffee & & \\

\bottomrule
\end{tabular}
}
\end{small}
\caption{\textbf{Imitation Learning Results for Long-Horizon Real-World Tasks.} The Success Rate (SR) is based on 10 trials, with SR-Subtask referring to subtask success rate.}
\label{tab:imitation_learning_lh}
\end{table}
